On spectral measures for certain unitary representations of R. Thompson's group F

The Hilbert space $\mathcal H$ of backward renormalisation of an anyonic quantum spin chain affords a unitary representation of Thompson's group $F$ via local scale transformations. Given a vector in the canonical dense subspace of $\mathcal H$ we show how to calculate the corresponding spectral measure for any element of $F$ and illustrate with some examples. Introducing the "essential part" of an element we show that the spectral measure of any vector in $\mathcal H$ is, apart from possibly finitely many eigenvalues, absolutely continuous with respect to Lebesgue measure. The same considerations and results hold for the Brown-Thompson groups $F_n$ (for which $F=F_2$).

==> foresttangle <==
#FIG 3.2  Produced by xfig version 3.2.5b
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 6975 1650 11325 4800
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 7650 4725 7650 3525 7050 1725
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7350 2550 7800 1725
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7650 3525 8700 1725
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9450 4725 9450 1725
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 10650 4725 10650 3525 10050 1725
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10650 3525 11250 1725
-6
6 225 1725 4575 4875
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 900 4800 900 3600 300 1800
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 600 2625 1050 1800
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 900 3600 1950 1800
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2700 4800 2700 1800
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 3900 4800 3900 3600 3300 1800
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3900 3600 4500 1800
-6
1 3 0 15 0 7 50 -1 20 0.000 1 0.0000 7650 3450 360 360 7650 3450 8010 3450
1 3 0 15 0 7 50 -1 20 0.000 1 0.0000 10650 3450 360 360 10650 3450 11010 3450
1 3 0 15 0 7 45 -1 20 0.000 1 0.0000 7350 2550 360 360 7350 2550 7710 2550
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	1 0 6.00 105.00 120.00
	 4650 3450 5325 3450
2 4 0 15 0 7 50 -1 -1 0.000 0 0 7 0 0 5
	 10875 5475 7350 5475 7350 4725 10875 4725 10875 5475
2 4 0 15 0 7 50 -1 -1 0.000 0 0 7 0 0 5
	 11475 5850 6675 5850 6675 1725 11475 1725 11475 5850
4 0 0 50 -1 0 30 0.0000 4 345 330 7500 3600 R\001
4 0 0 50 -1 0 30 0.0000 4 345 330 10500 3600 R\001
4 0 0 45 -1 0 30 0.0000 4 345 330 7200 2700 R\001

